Search for new phenomena in final states with an energetic jet and large missing transverse momentum in $pp$ collisions at $\sqrt{s}=13$ TeV using the ATLAS detector

Results of a search for new phenomena in final states with an energetic jet and large missing transverse momentum are reported. The search uses proton--proton collision data corresponding to an integrated luminosity of 3.2 fb${}^{-1}$ at $\sqrt{s}=13$ TeV collected in 2015 with the ATLAS detector at the Large Hadron Collider. Events are required to have at least one jet with a transverse momentum above 250 GeV and no leptons. Several signal regions are considered with increasing missing-transverse-momentum requirements between $E_{\rm T}^{\rm miss} >250$ GeV and $E_{\rm T}^{\rm miss} > 700$ GeV. Good agreement is observed between the number of events in data and Standard Model predictions. The results are translated into exclusion limits in models with large extra spatial dimensions, pair production of weakly interacting dark-matter candidates, and the production of supersymmetric particles in several compressed scenarios.

==> Makefile <==
# Makefile for creating an ATLAS LaTeX document
#------------------------------------------------------------------------------
# By default makes mydocument.pdf using target run_pdflatex.
# Replace mydocument with your main filename or add another target set.
# Adjust TEXLIVE if it is not correct, or pass it to "make new".
# Replace BIBTEX = bibtex with BIBTEX = biber if you use biber instead of bibtex.
# Adjust FIGSDIR for your figures directory tree.
# Adjust the %.pdf dependencies according to your directory structure.
# Use "make clean" to cleanup.
# Use "make cleanpdf" to delete $(BASENAME).pdf.
# "make cleanall" also deletes the PDF file $(BASENAME).pdf.
# Use "make cleanepstopdf" to rmeove PDF files created automatically from EPS files.
#   Note that FIGSDIR has to be set properly for this to work.

# If you have to run latex rather than pdflatex adjust the dependencies of %.dvi target
#   and use the command "make run_latex" to compile.
# Specify dvipdf or dvips as the run_latex dependency,
#   depending on which you want to use.

#-------------------------------------------------------------------------------
# Check which TeX Live installation you have with the command pdflatex --version
TEXLIVE  = 2013
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = bibtex
# BIBTEX = biber
DVIPS    = dvips
DVIPDF   = dvipdf

#-------------------------------------------------------------------------------
# The main document filename
BASENAME = mono_paper
#-------------------------------------------------------------------------------
# Adjust this according to your top-level figures directory
# This directory tree is used by the "make cleanepstopdf" command
FIGSDIR  = figs
#-------------------------------------------------------------------------------

# EPSTOPDFFILES = `find . -name \*eps-converted-to.pdf`
rwildcard=$(foreach d,$(wildcard $1*),$(call rwildcard,$d/,$2) $(filter $(subst *,%,$2),$d))
EPSTOPDFFILES = $(call rwildcard, $(FIGSDIR), *eps-converted-to.pdf)

# Default target - make mydocument.pdf with pdflatex
default: run_pdflatex

.PHONY: new newtexmf draftcover preprintcover auxmat \
	clean cleanpdf help

# Standard pdflatex target
run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

#-------------------------------------------------------------------------------
# Specify the tex and bib file dependencies for running pdflatex
# If your bib files are not in the main directory adjust this target accordingly
#%.pdf:	%.tex *.tex bibtex/bib/*.bib
%.pdf:	%.tex *.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<
#-------------------------------------------------------------------------------

new:
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed s/atlas-document/$(BASENAME)/ template/atlas-document.tex | \
	    sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME).tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  sed s/atlas-document/$(BASENAME)/ template/atlas-document.tex >$(BASENAME).tex; \
	fi
	cp template/atlas-document-metadata.tex $(BASENAME)-metadata.tex
	touch $(BASENAME).bib
	touch $(BASENAME)-defs.sty

newtexmf:
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed s/atlas-document/$(BASENAME)/ template/atlas-document-texmf.tex | \
	    sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME).tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  sed s/atlas-document/$(BASENAME)/ template/atlas-document.tex >$(BASENAME).tex; \
	fi
	cp template/atlas-document-metadata.tex $(BASENAME)-metadata.tex
	touch $(BASENAME).bib
	touch $(BASENAME)-defs.sty

draftcover:
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' template/atlas-draft-cover.tex \
	    >$(BASENAME)-draft-cover.tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  cp  template/$(BASENAME)-draft-cover.tex $(BASENAME)-draft-cover.tex; \
	fi

preprintcover:
	sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' template/atlas-preprint-cover.tex >$(BASENAME)-preprint-cover.tex
	#cp template/atlas-preprint-cover.tex $(BASENAME)-preprint-cover.tex

auxmat:
	sed s/atlas-document/$(BASENAME)/ template/atlas-auxmat.tex | \
	sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME)-auxmat.tex

run_latex: dvipdf

# Targets if you run latex instead of pdflatex
dvipdf:	$(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $(basename $<).pdf"

dvips:	$(BASENAME).dvi
	$(DVIPS) $<
	@echo "Made $(basename $<).ps"

# Specify dependencies for running latex
#%.dvi:	%.tex tex/*.tex bibtex/bib/*.bib
%.dvi:	%.tex *.tex *.bib
	$(LATEX)    $<
	-$(BIBTEX)  $(basename $<)
	$(LATEX)    $<
	$(LATEX)    $<

%.bbl:	%.tex *.bib
	$(LATEX) $<
	$(BIBTEX) $<

help:
	@echo "To create a new document give the commands:"
	@echo "make new [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "make"
	@echo "If your bib files are not in the main directory, adjust the %.pdf target accordingly." 
	@echo ""
	@echo "If atlaslatex is installed centrally, e.g. in ~/texmf:"
	@echo "make newtexmf [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo ""
	@echo "If you need a standalone draft cover give the commands:"
	@echo "make draftcover [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-draft-cover"
	@echo ""
	@echo "If you need a standalone preprint cover give the commands:"
	@echo "make preprintcover [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-preprint-cover"
	@echo ""
	@echo "If you need a document for auxiliary material give the commands:"
	@echo "make auxmat [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-auxmat"
	@echo ""
	@echo "make clean    to clean auxiliary files (not output PDF)"
	@echo "make cleanpdf to clean output PDF files"
	@echo "make cleanps  to clean output PS files"
	@echo "make cleanall to clean all files"
	@echo "make cleanepstopdf to clean PDF files automatically made from EPS"
	@echo ""

clean:
	-rm *.dvi *.toc *.aux *.log *.out \
		*.bbl *.blg *.brf *.bcf *-blx.bib *.run.xml \
		*.cb *.ind *.idx *.ilg *.inx \
		*.synctex.gz *~ ~* spellTmp 

cleanpdf:
	-rm $(BASENAME).pdf 
	-rm $(BASENAME)-draft-cover.pdf $(BASENAME)-preprint-cover.pdf
	-rm $(BASENAME)-auxmat.pdf

cleanps:
	-rm $(BASENAME).ps 
	-rm $(BASENAME)-draft-cover.ps $(BASENAME)-preprint-cover.ps
	-rm $(BASENAME)-auxmat.ps

cleanall: clean cleanpdf cleanps

# Clean the PDF files created automatically from EPS files
cleanepstopdf: $(EPSTOPDFFILES)
	@echo "Removing PDF files made automatically from EPS files"
	-rm $^

